Broadcast CONGEST Algorithms against Adversarial Edges

We consider the corner-stone broadcast task with an adaptive adversary that controls a fixed number of $t$ edges in the input communication graph. In this model, the adversary sees the entire communication in the network and the random coins of the nodes, while maliciously manipulating the messages sent through a set of $t$ edges (unknown to the nodes). Since the influential work of [Pease, Shostak and Lamport, JACM'80], broadcast algorithms against plentiful adversarial models have been studied in both theory and practice for over more than four decades. Despite this extensive research, there is no round efficient broadcast algorithm for general graphs in the CONGEST model of distributed computing. We provide the first round-efficient broadcast algorithms against adaptive edge adversaries. Our two key results for $n$-node graphs of diameter $D$ are as follows: 1. For $t=1$, there is a deterministic algorithm that solves the problem within $\widetilde{O}(D^2)$ rounds, provided that the graph is 3 edge-connected. This round complexity beats the natural barrier of $O(D^3)$ rounds, the existential lower bound on the maximal length of $3$ edge-disjoint paths between a given pair of nodes in $G$. This algorithm can be extended to a $\widetilde{O}(D^{O(t)})$-round algorithm against $t$ adversarial edges in $(2t+1)$ edge-connected graphs. 2. For expander graphs with minimum degree of $\Omega(t^2\log n)$, there is an improved broadcast algorithm with $O(t \log ^2 n)$ rounds against $t$ adversarial edges. This algorithm exploits the connectivity and conductance properties of G-subgraphs obtained by employing the Karger's edge sampling technique. Our algorithms mark a new connection between the areas of fault-tolerant network design and reliable distributed communication.

==> techniques-new-new.tex <==
\vspace{-5pt}
\section{Technical Overview}\label{sec:tech}
We start by considering the basic setting of handling a single adversarial edge $e'=(v_1,v_2)$. For simplicity, we will assume throughout that $m_0 \in \{0,1\}$, i.e. the broadcast message has a single bit. By having $O(\log n)$ repetitions, one can handle broadcast messages with $O(\log n)$ bits. 
A natural approach for broadcasting a message $m_0$ in the presence of an adversarial edge is to route the message along $3$-edge disjoint paths between the source vertex $s$, and each target vertex $v$. Since the adversarial edge appears on at most one of these paths, the correct message can be computed at each vertex $v$ by applying the majority vote. This basic approach has been applied in previous broadcast algorithms (e.g., \cite{Dolev82}) but has a few drawbacks. First, it assumes the knowledge of $3$ edge-disjoint paths between the source vertex $s$ and every other vertex $v$. Even in the fault-free setting, we have no round efficient algorithm for computing these paths. Secondly, for $D$-diameter graphs, these paths might have length $\Omega(D^3)$. Providing round-efficient algorithms in the \congest\ model, without assuming any global information (as in many of the prior works), calls for a new approach as we describe next. 




\vspace{-5pt}
\subsection{Adversarial Broadcast through Replacement-Path Covering}
The underlying objective in our broadcast algorithms is to exchange messages over reliable communication channels, free of the adversarial edge $e'$. There are two types of challenges: making sure that all the vertices first \emph{receive} the message $m_0$, and making sure that each vertex correctly \emph{distinguish} between the true bit and the false one. Our algorithm has two phases, a \emph{flooding} phase and an \emph{acceptance} phase, which at the high level, handles each of these challenges respectively. We first provide a high-level description of an $\widetilde{O}(D^3)$-round solution, and then explain how to improve it to $\widetilde{O}(D^2)$ rounds. 

\subsubsection{An $\widetilde{O}(D^2)$-Round Solution}
Our final algorithm employs a pipeline approach in which messages are propagated over each of the $G_i$ subgraphs in a round-by-round manner. Each message is indexed by the subgraph $G_i$ on which it should be propagated, and the messages are prioritized based on this index. Whereas pipeline is a quite common technique, especially in the context of broadcast, our implementation of it is quite nontrivial. Note that it is unclear how to apply the random-delay based scheduling schemes of~\cite{Ghaffari15,leighton1994packet} in our setting. Instead we propagate the messages over a collection of $G$-subgraphs $\mathcal{G}$ in a pipeline manner which, unless proven otherwise, might end in $\widetilde{O}(D^3)$ rounds, as will be illustrated next.
 
Our accepting mechanism explained above requires that every vertex $v$ receives the correct message over the subgraph $G_i$ that is good for $v$ (as defined above). The key challenge is in making sure that $v$ receives the message from $s$, indexed with subgraph $i$, within $\widetilde{O}(D^2)$ rounds. To see the challenge, let $P$ be some $s$-$v$ shortest path in $G_i$, and assume that all edges of $P$ appears only in the subgraph $G_i$ for $i=|\mathcal{G}|$. Since $s$ propagates the messages in a pipeline manner, $u$ receives the message $(m,i)$ from $s$ in round $i$. The complication arises in a situation where in that particular round $i$, $u$ also receive $\Omega(i)$ additional messages $(m',j)$ for $j<i$ which makes $(m,i)$ wait in the queue of $u$ for $\Omega(i)$ rounds (as we give priority based on the subgraph index). Such a delay for the $(m,i)$ message might occur on each of the $\Theta(D)$ edges of $P$, leading to a round complexity of $\Omega(D \cdot |\mathcal{G}|)$.
Note that this scenario might happen even in the fault-free setting, and has nothing to do with the behavior of the adversarial edge. In our analysis we show that such blocking events are bounded due to a special property of the covering family $\mathcal{G}$. 

The \emph{width} of the covering family $\mathcal{G}$, denoted as $\omega(\mathcal{G})$, is the largest number of subgraphs that avoid a given edge in $G$. For our selection of parameters, the construction of \cite{RPC21} provides a covering family $\mathcal{G}$ of width $\widetilde{O}(D)$. That is, every edge $e \in G$ appears on all the subgraphs of $\mathcal{G}$ except for $\widetilde{O}(D)$ many subgraphs.  Our analysis of the pipeline procedure then shows that each vertex $v$ receives the indexed messages $(m_0,i)$ within $O(D \cdot \omega(\mathcal{G})+|\mathcal{G}|)$ rounds. This in shown by providing the following counting argument. Let $P$ be some $s$-$v$ shortest path in $G_i$ (the subgraph that is good for $v$). Informally, we show that for each \emph{round} in which our message $(m_0,i)$ gets delayed in the queues of one of the vertices in $P$, there is one unique pair $(e'',j)$ that can be \emph{blamed} for that delay, where $e''$ is an edge on $P$ and $j<i$ is an index satisfying that $e'' \notin G_i$. Since the length of $P$ is bounded by $O(D)$ (as $G_i$ is good for $v$), and since the width $\omega(\mathcal{G})=\widetilde{O}(D)$, the total number of rounds in which the message $(m_0,i)$ gets delayed in the queues of $V(P)$ is bounded by $\widetilde{O}(D^2)$.  
To the best of our knowledge the width of covering families has played a role in the literature mainly in the context of obtaining fast query time in the setting of distance sensitivity oracles. We therefore find its impact on the round complexity of our broadcast algorithm to be quite extraordinary. 
%We next explain why sending this information is crucial to prevent a faulty acceptance. 
%
%\paragraph{Why should we send the path information?}
%Consider the following scenario where the graph $G$ contains an additional $v_1$-$v_2$ path $P=[v_1=x_1,\ldots, x_\ell=v_2]$ (i.e., between the endpoints of the adversarial edge). See Fig.~\ref{fig:bad-example}.
%Since the sampling of the adversarial edge might be inconsistent between its endpoints, in the first phase $v_1$ might receive a message originated from the adversary of $e'$ even in iterations in which $(v_1,v_2)$ is not sampled by $v_1$. For example, consider an iteration $i$ where $(v_1,v_2)\notin A_i(v_1)$, $(v_1,v_2)\in A_i(v_2)$ and every edge $(x_j,x_{j+1})\in P$ belongs to $A_i(x_{j+1})$. 
%
%\begin{wrapfigure}{r}{0.3\textwidth}
%\vspace{-15pt}
%\begin{center}
%\includegraphics[width=0.25\textwidth]{bad-example.pdf}
%\end{center}
%\vspace{-10pt}
%\caption{\small{Illustrating the key challenge in reducing the running time to $\widetilde{O}(D)$ in the presence of a adversarial edge.}\label{fig:bad-example}}
%%	\vspace{-10pt}
%\end{wrapfigure} 
%
%Since $(v_1,v_2)\in A_i(v_2)$, the node $v_2$ might receive a faulty message from the adversary and propagate it to $v_1$ over the path $P$. Consequently, $v_1$ ends up receiving a false message originated by an edge that is not part of the current communication graph from its point of view. This is clearly avoided when sending path information, as in the latter case $v_1$ can learn that $(v_1,v_2)$ was part of this path. %and ignore that message \textbf{YH: why should he ignore the message?}.  
%As we discuss later on in Sec. \ref{sec:opt} the propagation of the path information can be omitted when the adversary is symmetric (restricted to send the same faulty messages to both of the edge endpoints). In the latter cases, we can indeed provide an $\widetilde{O}(D)$ round algorithm for the problem. 
%
%%
%%Note that this above-mentioned scenario could also be avoided provided that the sampling of the edges into each subgraph $G_i$ is consistent between its endpoints. This boils down into a \emph{Collective Coin Flipping} problem\footnote{In that problem, vertices need to agree on a single random bit.}\cite{ben1989collective}, however, it is unclear how to solve this take in $o(D^2)$ rounds. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Broadcast without Knowing the Diameter}\label{sec:notknowing}
The computation of the covering family requires the knowledge of $D$ (or any linear estimate of that). 
Approximating the diameter in the adversarial setting seems, at first glance, to be just as challenging as the broadcast task itself. To mitigate this barrier, we take the following approach. 
Let $\cA$ be the broadcast algorithm that runs based on some given diameter estimate $\widehat{D}$ known to all vertices. Algorithm $\cA$ runs for a fixed number of $\widetilde{O}(\widehat{D}^2)$ rounds. Our algorithm makes $\ell = (\log D)$ applications of algorithm $\cA$, where in the $i$'th application, it implements $\cA$ with a diameter guess $\widehat{D}=2^i$. Since the algorithm does not know $D$, it is required that after $\ell$ applications, all vertices will accept the broadcast message and terminate. While this guessing approach is quite straightforward in the standard non-adversarial distributed setting, its implementation in our setting is not that trivial. 
Intuitively, as long as $\widehat{D}<D$, there must be some vertices in the graph that still did not accept any message (or even just received any message) from $s$. To make sure the network proceeds to the next diameter guess, we would like these uninformed vertices $v$ to inform $s$ (and the rest of the vertices). This, however, appears at first sight to be just as hard as the broadcast task again! That is, while the algorithm failed to inform $v$ on the correct message from $s$ (i.e., failed in establishing a realizable channel from $s$ to $v$), we need to form such a channel in the reverse direction.
The key and somewhat surprising observation is that this task is in fact simpler. To see this, consider the $i$'th application of $\cA$ with diameter guess $\widehat{D}=2^i<D$, let $N$ be the subset of vertices that still did not accept any message at the end of $\cA$, and let $R=V \setminus N$ be the set of vertices that already accept the message from $s$. Clearly, $s \in R$, and $\dist_G(s, R)=\max_{r \in R}\dist_G(s,r) \leq \widehat{D}$. In addition, since the graph is $3$-edge connected, the $(N,R)$ cut value is at least $3$. Altogether, we get that the graph $G'$ obtained by contracting \footnote{I.e., we contract all edges with both endpoints in $N$.} all vertices in $N$ into a single vertex $a$, satisfies the following: (i) it is $3$-edge connected, (ii) it contains $s$ and (iii) it has diameter $O(\widehat{D})$. Therefore, applying the broadcast algorithm on $G'$ with the guess $\widehat{D}$ (i.e., the correct diameter bound of $G'$) and with a source vertex $a$ allows all vertices in the graph to know that $\widehat{D}<D$ and to proceed to the next guess value.  This graph contraction is only used here to provide an illustrative description of the algorithm. In the actual algorithm, the contraction effect is obtained by letting all vertices in $N$ act as senders in the broadcast algorithm $\cA$ applied on $G$ with input diameter $\widehat{D}$. 


%\subsection{Broadcast with Multiple Adversarial Faults}
%Finally, we consider the complexity of the problem with $t$ adversarial edges (and vertices). On the positive side, we can show that the algorithm of Theorem \ref{lem:broadcast} extends to multiple faults, at the expense of having a round complexity of $(t D \log n)^{O(t)}$. In the same manner, for $t$ adversarial vertices, we can provide an algorithm with $(t\Delta\cdot D \log n)^{O(t)}$ rounds, where $\Delta$ is the maximum degree of the graph. Our vertex extension only holds provided that the source is reliable.  
%These extensions are based on the observation that in every $D$-diameter $(2t+1)$-edge (vertices) connected graph, for any set $F$ of at most $2t$ edges (vertices) , the diameter of the graph $G \setminus F$ is bounded by $O(t D)$ (resp., $O(t \Delta D)$). From now on, we focus on the case of adversarial edges. 
%%sequence of at most $2t$ faults $F$, the diameter of the graph is bounded by $O(t D)$.
%Our upper bound algorithm floods messages over the subgraphs of an $(L,2t)$ covering family $\mathcal{G}$ for $L=O(tD)$. The size of this covering family is $(t D\log n)^{O(t)}$. The messages exchanged over each subgraph $G_i$ also contain the path information along which the message has been received. Despite the fact that all these paths have length $O(t D)$, the final round complexity of the algorithm is dominated by the cardinality of $\mathcal{G}$. 
%The acceptance rule is also modified, where a given message $m$ is accepted by a given target $v$ only if the 
%$s$-$v$ paths along the message $m$ has been received has a sufficiently large $s$-$v$ cut.
%
%
%
%% 
%We then turn to consider the lower bound aspects of the problem. Towards that goal we provide 
%a graph-theoretical characterization of route-sets of large flows. For a pair of vertices $s,v$, a route-set $\mathcal{P}_{s,v}$ is a collection of $s$-$v$ paths of sufficiently large total flow. Specifically, in our case, we consider route-sets of total integral flow at least $t+1$. In other words, we consider a collection of $s$-$v$ paths 
%$\cP_{s,v}$ such that the min-cut between $s$ and $v$ in the union of these paths is at least $t+1$. Our upper bound routes messages along such paths using covering families. The paths formed by this technique have length $O(t D)$ but their edge overlap might be as large as $D^{\Omega(t)}$. Since in every round, we can send at most $O(\log n)$ bits of information, having $D^{\Omega(t)}$ paths that pass through the same edge lead to our round complexity of $(D/t)^{\Omega(t)}$ rounds. We define the congestion and dilation of a route-set $\cP_{s,v}$ by:
%$$\congestion(\cP_{s,v})= \max_{e \in E}|\{P \in \cP_{s,v} ~\mid~ e \in P\}| \mbox{~~and~~} \dilation(\cP_{s,v})= \max_{P \in \cP_{s,v}}|P|~.$$
%\vspace{-7pt}
%\begin{question}\label{q:route}
%Is it possible to route messages on $s$-$v$ paths that have simultaneously both small length (i.e., dilation) and bounded overlap (i.e., congestion)?
%\end{question}\vspace{-7pt}
%Unfortunately, we show the answer to Q. \ref{q:route} is NO when $D>t$. For every $D>t$, we present a construction of $(2t+1)$-edge connected graph $G$ for which there exists a pair of vertices $s,v$ such that for any route set $\cP_{s,v}$ with flow at least $t+1$, it holds that
%$$\congestion(\cP_{s,v})+\dilation(\cP_{s,v})= (D/t)^{\Omega(t)}.$$
%This in particular implies that the route-sets obtained by the FT-sampling technique are, in fact, existentially \emph{optimal} in terms of their congestion+dilation value. 
%Using this characterization, we are able to provide a lower-bound of $(D/t)^{\Omega(t)}$ for the complexity of the problem against $t$ adversarial edges. This lower bound holds for a restricted class of store-and-forward algorithms which still capture many of the existing broadcast algorithms with adversarial faults. 
%The high-level idea of the argument is as follows. Let $G_t$ be a graph in which there exists an $s$-$v$ pair whose route-set $\mathcal{P}_{s,v}$ satisfies that $\congestion(\cP_{s,v})+\dilation(\cP_{s,v})= (D/t)^{\Omega(t)}$. 
%Let $\mathcal{A}$ be a store-and-forward algorithm, and for simplicity assume that it is deterministic. We also assume that  $\mathcal{A}$ is input-invariant, i.e., its behavior does not depend on the content of the message $m_0$. We then consider the execution of $\cA$ when $m_0=0$ (resp., $m_0=1$) and when all edges in the execution behaved in a reliable manner. Denote this execution by $\mathcal{E}_0$ (resp., $\mathcal{E}_1$). 
%Let $\mathcal{P}_{s,v}$ be the set of paths along which the messages from $s$ arrive to $v$ in the execution $\mathcal{E}_0$. Since the algorithm is input-invariant, the same set of paths have been used in $\mathcal{E}_1$ as well. The key argument is to show that the $s$-$v$ flow of the route-set $\cP_{s,v}$ is at least $t+1$. To see this, assume towards contradiction that there is a set of at most $t$ edges $F'$ that disconnect $s$ and $v$ in $\bigcup_{P \in \cP_{s,v}}E(P)$. Let $\mathcal{E}'$ be an execution in which $m_0=0$ and all edges of $F'$ are adversarial. During the execution, each adversarial edge $e' \in F'$ sends the same messages that $e'$ sends in the execution $\mathcal{E}_1$, i.e., when $m_0=1$. Since this occurs on all cut edges $F'$, the views of $v$ in $\mathcal{E}'$ and in $\mathcal{E}_1$ are identical, and $v$ accepts $m'=1$, leading to a contradiction. We conclude that the $s$-$v$ flow in $\cP_{s,v}$ is at least $t+1$ and thus 
%$\congestion(\cP_{s,v})+\dilation(\cP_{s,v})= (D/t)^{\Omega(t)}$.  Since $\cA$ is a store-and-forward algorithm, every edge $e \in P$ for $P \in \cP_{s,v}$ must forward all the messages for each of the paths it belongs to, leading to a round complexity of $(D/t)^{\Omega(t)}$.

%
%\yael{Now that we do not have the lower bound I wander if we should include the t faults in the tech overview}
%
%\yael{We can 're-live' the subsection regarding optimal broadcast.}
%\vspace{-10pt}
%\subsection{Optimal Broadcast Algorithms with Shared Randomness}\label{sec:opt}
%To gain a better understanding of the complexity of the problem as well as to underlie the key barriers for achieving $\widetilde{O}(D)$ solutions, we consider the problem in relaxed settings, such as having a shared seed of $\widetilde{O}(1)$ bits with all vertices.
%%The common feature of all these settings is that they provide some sort of consistency between the endpoints of the adversarial edge.  For example, in the symmetric adversary setting, this consistency is obtained by forcing the adversary to send the same message to both endpoints. 
%In the shared randomness setting it is obtained by sharing $\widetilde{O}(1)$ bits with all vertices. We note that for general number of faults $t$, these relaxations, can at best improve the broadcast algorithm by a factor of $D$. It would be very interesting to consider weaker adversaries under which the exponential dependency in $t$ can be eliminated. 
%\vspace{-5pt}
%\paragraph{Optimal algorithm with a symmetric adversary.} Our algorithm is based on using a covering family with improved size and width bounds. This family can be computed by applying a directed variant of the FT-sampling technique. Specifically, the first phase propagates messages over $G_i$ subgraphs, where each $G_i$ is a directed graph defined by letting each vertex $v$ locally sample each of its incoming edges in $G_i$, by sampling each of its $G$ edges independently with probability of $1-1/D$. We show that flooding the messages along this directed graph collection is sufficient in order to determine the correct broadcast message. 
%The nearly optimal Broadcast algorithm for these settings still follows the two-phase structure described above. The key modification is that the first phase implements a light-variant of the flooding algorithm in which the messages exchanged over each sampled subgraphs $G_i$ for $i \in \{1,\ldots, r\}$ are sent in a pipeline manner.\textbf{YH: We note that in the Byzantine setting it is unclear whether one can apply efficient scheduling schemes such as ~\cite{Ghaffari15,LeightonMR94}.}
% Importantly, the path information that was attached to each message in our original algorithm is now omitted. 
%The nearly optimal broadcast algorithms for these settings still follows the two-phase structure described above. The key modification is that the first phase implements a light-variant of the flooding algorithm in which the path information that was attached to each message in our original algorithm is now omitted.
%Additionally, the messages exchanged over each sampled subgraphs $G_i$ for $i \in \{1,\ldots, r\}$ are sent in a pipeline manner. We note that in the adversarial setting it is unclear how to apply the nearly optimal scheduling schemes of~\cite{Ghaffari15,LeightonMR94}.
%The implementation of the second phase slightly differs in each of the settings. The correctness argument has two main pieces.  The key challenge is to show that the light-variant can be implemented within $\widetilde{O}(D)$ rounds. Here we use the useful property of the FT-sampling procedure in which every edge $e$ can be shown to appear w.h.p in all \emph{but} $O(\log n)$ sampled subgraphs. This plays a critical role in the round complexity argument, and it is independent of the properties of the adversary considered. 
%The second part of the argument exploits the properties of the adversary to show that all vertices accept the correct message. 

